Summary Report for Snowmass Community Engagement Frontier Topical Group 06: Public Policy & Government Engagement

This document is the Snowmass summary report for the Public Policy & Government Engagement topical group within the Community Engagement Frontier. This report discusses how the U.S. High Energy Physics (HEP) community currently engages with government at all levels and provides recommendations for how the execution of these actives can be improved and for how the scope of existing activities can be expanded. This includes the current HEP Congressional government engagement "DC trip", materials produced for communication with government officials, government engagement in areas other than HEP funding, and interactions with the funding agencies, Executive Office of the President, and state and local governments.

==> findings/finding1.tex <==
\textbf{Finding - There is not consensus on how best to proceed in this area} \textcolor{red}{this has to be standalone sentence - not convinced it cant just be in the text}

\textit{During the course of proceedings of this topical group, no consensus was reached on how best to meaningfully engage in the advocacy for topics affecting our field beyond HEP funding.}
